GenAI Assisting Medical Training

Medical procedures such as venipuncture and cannulation are essential for nurses and require precise skills. Learning this skill, in turn, is a challenge for educators due to the number of teachers per class and the complexity of the task. The study aims to help students with skill acquisition and alleviate the educator's workload by integrating generative AI methods to provide real-time feedback on medical procedures such as venipuncture and cannulation.

==> backup.tex <==
\item \textbf{Dataset Processing:}
    \begin{enumerate}
    
    \item \textbf{Participant and Procedure Details:} Collection during 3 days (27.-29.11.2023) at Southampton university, two procedures (cannulation and venipuncture), 20 participants (13 students with different levels of experience, 7 experts). Each participant performed each procedure twice, i.e., 80 recordings in total. The dataset consists of:
        \begin{itemize}
            \item 3 static cameras placed at the foot, head, and side of the bed
            \item 1 GoPro camera
            \item All cameras recorded in 1920x1080 resolution at 60 Hz
            \item Audio recordings from the video cameras
            \item IMU data from 2 Apple smartwatches placed on the left and right wrists of the participants
            \item Feedback forms filled in by professional experts/observers during the participants’ performance of the procedure
            \item Audio recordings of feedback given by observers to the participants directly after they performed the procedure
        \end{itemize}

